A Roadmap For Scientific Ballooning 2020-2030

From 2018 to 2020, the Scientific Balloon Roadmap Program Analysis Group (Balloon Roadmap PAG) served as an community-based, interdisciplinary forum for soliciting and coordinating community analysis and input in support of the NASA Scientific Balloon Program. The Balloon Roadmap PAG was tasked with articulating and prioritizing the key science drivers and needed capabilities of the Balloon Program for the next decade. Additionally, the Balloon Roadmap PAG was asked to evaluate the potential for achieving science goals and maturing technologies of the Science Mission Directorate, evaluate the Balloon Program goals towards community outreach, and asses commercial balloon launch opportunities. The culmination of this work has been a written report submitted to the NASA Astrophysics Division Director.

==> Old_Files/Bibliography.tex <==
\begin{thebibliography}{80}

\bibitem{PAG-letter} A copy of the PAG letter is available at 
\url{https://www.phys.hawaii.edu/~gorham/Post/Roadmap2018/BalloonRoadmappers.html}.

\bibitem{PAG-Report} The current draft of the PAG report is available at \url{https://www.phys.hawaii.edu/~gorham/Post/Roadmap2018/BalloonRoadmapDraft.pdf}.
In addition, a compilation of relevant documents and community input can be found at 
\url{https://www.phys.hawaii.edu/~gorham/Post/Roadmap2018/BalloonRoadmappers.html}.

\bibitem{Batalha2018}

\bibitem{Parmentier2019}

\bibitem{Centennial_of_flight1} 
\url{https://www.centennialofflight.net/essay/Lighter_than_air/Science_Missions-20th-Part_II/LTA15.htm}.

\bibitem{Crouch83}
Crouch, Tom D., The Eagle Aloft: Two Centuries of the Balloon in America. Washington, D.C.: Smithsonian Institution Press, 1983.

\bibitem{Kirshner85}
Kirschner, Edwin J., Aerospace Balloons – From Montgolfiere to Space. Fallbrook, Calif.: Aero Publishers, Inc. 1985.

\bibitem{Payne91}
Payne, Lee. Lighter Than Air: An Illustrated History of the Airship. N.Y.: Orion Books, 1991.

\bibitem{Hess28}
Hess, Victor F. (1928). The Electrical Conductivity of the Atmosphere and Its Causes. Constable \& Company. 

\bibitem{Rossi64}
Rossi, Bruno. Cosmic Rays. N.Y.: Wiley \& Sons, 1964.


\bibitem{Abbot44}
Abbot, Charles Greeley. The Sun and the Welfare of Man. N.Y.: Smithsonian Institution Series, 1944.

\bibitem{vanAllen} \url{http://www-pw.physics.uiowa.edu/van90/McIlwain_lecture.pdf}.

\bibitem{Stratoscope} Suomi, V. E and Beson, E. E. Astronomical Observations from a Skyhook Balloon. Winzen Research, Inc. Technical report 1150-R, February 1955; Rogerson, John B. Jr. (January 1958). "Project Stratoscope -- Solar Photographs from 80,000 Feet". Sky and Telescope. 17. p. 112.

\bibitem{IC79} M. G. Aartsen et al., Phys. Rev. Lett 117, 241101 (2016).

\bibitem{A4neutrino}
Constraints on the ultra-high energy cosmic neutrino flux from the fourth flight of ANITA,
P. W. Gorham, et al. [ANITA collaboration] (2019), arXiv:1902.04005.

\bibitem{ANITA_CR}S. Hoover \emph{et al},  [ANITA collaboration], \emph{Observation of Ultra-high-Energy CRs with the 
ANITA Balloon-Borne Radio Interferometer}, 
Phys. Rev. Lett. {\bf{105}}, (2010).

\bibitem{Upshowers} P. W. Gorham {\it et al.} [ANITA Collaboration], 
Characteristics of Four Upward-pointing Cosmic-ray-like Events Observed with ANITA,
Phys. Rev. Lett. (2016), 117, 071101, \url{http://arxiv.org/abs/1603.05218}

\bibitem{A3upwardshower} P. Gorham, \emph{ et al. } [ANITA Collaboration],  
``Observation of an Unusual Upward-going Cosmic-ray-like Event in the Third Flight of ANITA,''
Phys. Rev. Lett. 121, 161102 (2018)
DOI:	10.1103/PhysRevLett.121.161102, 
\url{ https://arxiv.org/abs/1803.05088 }.

\bibitem{A4CRs} P. W. Gorham, {\it et al.} [ANITA collaboration], Ultra-high Energy Air Showers Observed by ANITA-IV,
Phys. Rev. Lett. 2020, in press.;
\url{https://arxiv.org/abs/2008.05690}.

\bibitem{PUEO} PUEO is described in ``Searches for Ultra-High Energy Neutrinos with ANITA,''
C. Deaconu for the ANITA Collaboration, 
 PoS ICRC2019 (2020) 867.
 
\bibitem{Besson12} D. Besson, R. Dagkesamanskii, E. Kravchenko, I. Kravchenko, I. Zheleznykh,
Tethered balloons for radio detection of ultra high energy cosmic neutrinos in Antarctica,
Nuclear Instruments and Methods in Physics Research Section A: Accelerators, Spectrometers, Detectors and Associated Equipment,
Volume 662, Supplement 1,
2012,
Pages S50-S53,
ISSN 0168-9002,
https://doi.org/10.1016/j.nima.2010.11.046.

\bibitem{Cosmin20} C. Deaconu, 2020, personal communication.

\bibitem{Walker-book} C. Walker, Terahertz Astronomy, 2016, (CRC Press: Boca Raton, FL).

	
\bibitem{schonfelder1993} {Instrument Description and Performance of the Imaging Gamma-Ray Telescope COMPTEL Aboard the Compton Gamma-Ray Observatory},
{V. Sch\"{o}nfelder and H. Aarts and K. Bennett and H. de Boer and J. Clear and W. Collmar and A. Connors and A. Deerenberg 
	and R. Diehl and A. von Dordrecht and J. W. den Herder and W. Hermsen and M. Kippen and L. Kuiper and G. Lichti and J. Lockwood and J. 
	Marci and M. McConnell and D. Morris and R. Much and J. Ryan and G. Simpson and M. Snelling and G. Stacy and H. Steinle and A. Strong 
	and B. N. Swanenburg and B. Taylor and C. de Vries and C. Winkler},
	Ap. J. Suppl. 86, 657, 1993.

\bibitem{kierans2016}The 2016 Super Pressure Balloon flight of the Compton Spectrometer and Imager,.
{{Kierans}, C.~A. and {Boggs}, S.~E. and {Chiu}, J.-L. and {Lowell}, A. and {Sleator}, C. and {Tomsick}, J.~A. and {Zoglauer}, 
	A. and {Amman}, M. and {Chang}, H.-K. and {Tseng}, C.-H. and {Yang}, C.-Y. and {Lin}, C.-H. and {Jean}, P. and {von Ballmoos}, P.},
	Gamma-Ray Astrophysics in Multi-Wavelength Perspective, Proceedings in 11th INTEGRAL Conference, 2016.

\bibitem{ueno2012} Development of the balloon-borne sub-MeV gamma-ray Compton camera using an electron-tracking gaseous TPC and a scintillation camera,
{K. Ueno and T. Mizumoto and K. Hattori and N. Higashi and S. Iwaki and S. Kabuki and Y. Kishimoto and S. Komura and H. Kubo and S. Kurosawa},
{Journal of Instrumentation} 7, 1088, 2012.

\bibitem{Bloser2018}{The Advanced Scintillator Compton Telescope (ASCOT) balloon payload}, 
{ P. F. Bloser,T. Sharma,J. S. Legere,C. M. Bancroft,M. L. McConnell,J. M. Ryan,A. M. Wright},
\url{https://doi.org/10.1117/12.2312150}, 2018; \url{https://ui.adsabs.harvard.edu/abs/2018Galax...6...30F}.


\bibitem{2018Galax}The PoGO+ Ballon-Borne Hard X-ray Polarimetry Mission, 
{Friis}, M. and {Kiss}, M. and {Mikhalev}, V. and {Pearce}, M. and 
	{Takahashi}, H., arxiv:1803.02106, 2018.


\bibitem{mcconnell2018} The continued development of a low energy Compton imager for GRB polarization studies,
Mark L. McConnell,Peter F. Bloser,Jason S. Legere,James M. Ryan,Lorraine Hanlon,Sheila McBreen,Alexey Uliyanov,
Proceedings Volume 10699, Space Telescopes and Instrumentation 2018: Ultraviolet to Gamma Ray; 
SPIE Astronomical Telescopes + Instrumentation, 2018, Austin, Texas, United States, 2018.

\bibitem{xcal2019}Results From the Antarctic Balloon Flight of the Hard X-ray Polarimeter X-Calibur,
{{Kislat}, F. and {Abarr}, Q. and {Bose}, R. and {Braun}, D. and 
	{de Geronimo}, G. and {Dowkontt}, P. and {Errando}, M. and {Gadson}, T.~A. and 
	{Guarino}, V. and {Heatwole}, S.~E. and {Iyer}, N. and {Kiss}, M. and 
	{Kitaguchi}, T. and {Krawczynski}, H. and {Kushwah}, R. and 
	{Lanzi}, J. and {Li}, S. and {Lisalda}, L. and {Okajima}, T. and 
	{Pearce}, M. and {Peterson}, Z. and {Rauch}, B. and {Stuchlik}, D. and 
	{Takahashi}, H. and {Tang}, J. and {Uchida}, N. and {West}, A.
	},{American Astronomical Society Meeting Abstracts},2019, \url{https://ui.adsabs.harvard.edu/abs/2019AAS...23421508K}



\bibitem{Hinode} Committee on NASA's suborbital research capabilities, N. R. C. (2010). Revitalizing NASA's Suborbital Program: 
 Advancing Science, Driving Innovation, and Developing a Workforce. The National Academies Press, Washington, D. C.

% \bibitem{SUNRISE} Solanki, S. K., Barthol, P., Danilovic, S., Feller, A., Gandorfer, A., Hirzberger, J., Riethmu ̈ller, 
% T. L., Schu ̈ssler, M., Bonet, J. A., Mart ́ınez Pillet, V., del Toro Iniesta, J. C., Domingo, V., Palacios, 
% J., Kno ̈lker, M., Bello Gonza ́lez, N., Berkefeld, T., Franz, M., Schmidt, W., and Title, A. M. (2010). 
% SUNRISE: Instrument, Mission, Data, and First Results. Astrophys. J. Lett., 723:L127–L133.

\bibitem{Anderson64} Anderson, K. A., and Milton, D. W. ( 1964), 
Balloon observations of X rays in the auroral zone: 3. High time resolution studies, J. Geophys. Res., 69( 21), 4457-4479, doi:10.1029/JZ069i021p04457.


%% Exoplanets & Stellar Astro references
% Batalha, N., Smith, A., Lewis, N., Marley, M., Fortney, J. and Macintosh, B., 2006, Astron.
% J., 156, https://doi.org/10.3847/1538-3881/aad59d .
% Bryden, G., Beichman, C. A., Trilling, D. E., et al., 2006, Ap. J., 636 (2006): 1098–1113.
% Eiroa, C et al., 2013, A&A, 555, A11 Engelke, C. W., Price, S. D., & Kraemer, K. E. 2010, AJ,
% 140, 1919
% Gao, P., Marley, M. S., Zahnle, K., Robinson, T. D., & Lewis, N. K. 2017, AJ, 153, 139
% Greaves, J. S et al., 2005, Ap. J., 619 (2005): L187– L190.
% Kalas, P., Fitzgerald, M. P., and Graham, J. R., 2007, Ap. J., 661, L85 (2007).
% Lupu, R. E., Marley, M. S., Lewis, N., et al. 2016, AJ, 152, 217
% Mayorga, L. C., Jackiewicz, J., Rages, K., et al. 2016, AJ, 152, 209
% Nayak, M., Lupu, R., Marley, M. S., et al. 2017, PASP, 129, 034401
% Parmentier V,. and Crossfield I. J. M., doi: 10.1007/978-3-319-55333-7_116

\bibitem{EPO1}	Walker, R.S., Peters, F.W., Aldrin, B., et al., “Final Report of the Commission on the Future of the United States Aerospace Industry”, Crystal Gateway 1, Suite 940, 1235 Jefferson Davis Highway, Arlington, Virginia 22202, 2002,
	\url{http://ita.doc.gov/td/aerospace/aerospacecommission/aerospacecommission.htm}

\bibitem{EPO2}	Aldridge, E.C. Jr., Fiorina, C.S., Jackson, M.P., Leshin, L.A., Lyles, L.L., Spudis, P.D., Tyson, N.D., Walker, R.S., and Zuber, M.T., “Report of the President’s Commission on Implementation of United State Space Exploration Policy”, ISBN 0-16-073075-9, Superintendent of Documents, U.S. Government Printing Office, Mail Stop SSOP, Washington, DC 20402-001, 2004

\bibitem{EPO3}	Augustine, N.R. et al., “Rising Above the Gathering Storm, Revisited”, National Academy of Sciences, National Academy of Engineering, and Institution of Medicine of the National Academies, National Academies Press, Washington, DC. 2010, \url{https://www.nap.edu/catalog/12999/rising-above-the-gathering-storm-revisited-rapidly-approaching-category-5}

\bibitem{EPO4}	“Building the Space Workforce of the Future: STEM Engagement for a 21st Century Education”, Hearing before the U.S. Senate Committee on Commerce, Science, and Transportation, November 5, 2019, \url{https://www.commerce.senate.gov/2019/11/building-nasa-s-workforce-of-the-future-stem-engagement-for-a-21st-century-education}

\bibitem{EPO5}		“Charting a Course for Success: America’s Strategy for STEM Education”, A Report by the Committee on STEM Education of the National Science \& Technology Council, The White House, December 2018, \url{https://www.whitehouse.gov/wp-content/uploads/2018/12/STEM-Education-Strategic-Plan-2018.pdf}

\bibitem{EPO6}		“NASA Strategic Plan 2018”, National Aeronautics and Space Administration, 2018, 
\url{https://www.nasa.gov/sites/default/files/atoms/files/nasa_2018_strategic_plan.pdf}

\bibitem{EPO7}	“Explore Science 2020-2024”, National Aeronautics and Space Administration, Science Mission Directorate, 2020, \url{https://science.nasa.gov/about-us/science-strategy}

\bibitem{EPO8}	Letter from Dr. Angela Des Jardins, Submitted to the Balloon Roadmap Program Analysis Group, November 2018

\bibitem{EPO9}	“Cubes in Space: Ingenuity taking flight”, website https://www.cubesinspace.com/, 2019

\bibitem{EPO10}		“Automatic Packet Reporting System”, B. Bruninga, website http://www.aprs.org/

\bibitem{EPO11}	Undergraduate Student Instrument Project (USIP) Student Flight Research Opportunity (SFRO), NASA solicitation NNH15ZDA010C, \url{https://nspires.nasaprs.com/external/solicitations/summary.do?method=init&solId={FABD5D3A-878E-A99F-5D05-87AAD356CC9E}&path=closedPast} , 2015

\bibitem{EPO12}	“The High Altitude Student Platform (HASP) as a Model Multi-Payload Balloon Platform”, T.G. Guzik for the HASP Collaboration, 2015 IEEE Aerospace Conference, 10.1109/AERO 2015.7118985 March 7-14, 2015, Big Sky, MT (2015)

\bibitem{EPO13}	“Eclipse Ballooning Project Live Streaming Activity: Overview, Outcomes, and Lessons Learned”, Angela Colman Des Jardins et al., Celebrating the 2017 Great American Eclipse: Lessons Learned from the Path of Totality, ASP Conference Series, Vol. 516, Sanlyn Buxner, Linda Shore, and Joseph Jensen, eds., Astronomical Society of the Pacific, 2019

\bibitem{EPO14}	“Possibilities for STEM engagement in the Nationwide Eclipse Ballooning Project 2021-2025”, R.M. Larimer, 2020 Academic High Altitude Conference, September 19,2020

\bibitem{EPO15}	“Stratospheric Balloons as a Low-Cost Vehicle for Sustained Student Engagement and Aerospace Workforce Development”, J. Hoover and J. Acevedo, White paper submitted to the Balloon Roadmap Program Analysis Group, November 2018


\end{thebibliography}

==> Old_Files/Earth_Science_new.tex <==

\section{Earth Science}
\label{sec:earth}



% \begin{tcolorbox}[colback=royalblue!8!white,colframe=royalblue,fonttitle=\bfseries,title=Relevance to SMD Science Goals]

% Currently, NASA-supported Earth Science remote sensing studies primarily use aircraft or satellite observations. However, balloons provide a unique platform for observations in remote locations such as Antarctica and for in-situ studies the Earth's atmosphere. 

% ADD -  BIG questions in Earth science?
%  \textit{????} and \textit{????}

% \vspace{0.75cm}

% \textbf{Climate Change} (Sec.~\ref{sec:climate}) .... as stated in Section~..... of NASA's ????? Roadmap: 
% \begin{quote}
% The blah.
% \end{quote}
% The studies of ???, \textit{????}, through ???.

% \vspace{0.75cm}

% Studies of \textbf{Stratospheric Ozone Loss} (Sec.~\ref{sec:ozone}) directly addresses the question \textit{???} posed in ???? \textbf{Impact of Solar Radiation on the Stratosphere} (Sec.~\ref{sec:radiation_budget} answers \textit{??}

% \vspace{0.75cm}

% \textbf{High Energy Atmospheric Physics} (Sec.~\ref{sec:TGF}), a relatively young field....


% \end{tcolorbox}


\subsection{Introduction: Rapid Changes in the Earth’s Climate Structure}

There is a critical need for fundamental advances in climate observations for quantitative risk forecasting – an advanced generation of very high spatial resolution three-dimensional observations for which scientific balloon observations are of critical importance. Events, rather than scientific breakthroughs have increasingly dominated our collective awareness of the risks associated with rapid, irreversible changes to the Earth’s climate structure. In particular: the rate of ice volume loss from the glacial structures of Greenland and the West Antarctic that controls the rate of sea level rise; rapid increases in the frequency, intensity and geographic extent of wild fires, of severe storms with associated losses of life and property, of coastal and inland flooding, of increases in UV radiation over the central United States in summer, and of greater severity of agricultural drought and deadly heat waves.

The inability to accurately forecast the rate of onset of these irreversible changes to the climate system that will destabilize society in the coming decades, underscores the current large uncertainties in quantitative forecasting. This in turn directly implies that we have lost control of the ability to quantitatively navigate the risks associated with rapid, irreversible changes to the Earth’s climate structure as the future unfolds. Scientific balloon observations constitute an integral part of strategic innovations in climate research and associated advances in public policy.

There is a fundamental reason why tested and trusted quantitative forecasts of risk associated with increased forcing of the climate by CO2 and CH4 are unavailable. Simultaneous, high spatial resolution, observations of the interdependent variables that control the mechanistically coupled climate system are of critical importance for quantitative forecasting. Yet the critically needed array of high spatial resolution, three dimensional observations, determined simultaneously within the same volume element of each of the climate structures, are not available. This requires a new generation of advanced technology associated with scientific ballooning.

We consider here four first order scientific challenges that a new generation of balloon-borne stratospheric observing systems can address: 
    1. Changes to the large-scale dynamical structure of the Earth’s climate system resulting from the continued use of fossil fuels,
    2. Stratospheric ozone loss over the central United States in summer resulting from increasing frequency and intensity of convective storm systems over the Great Plains driven by Climate Change,
    3. Increased global loss of stratospheric ozone resulting from climate change induced increases in lower stratospheric water vapor, decreases in lower stratospheric temperatures, and the convective injection of chlorine and bromine radical precursors from the boundary layer, and
    4. Advances in geoengineering of the climate via solar radiation management (SRM).
    
We briefly introduce here the StratoCruiser system that offers transformational advances in climate research focused on the development of quantitative forecasts of climate risk. The StratoCruiser observing system displayed in Figure 1 provides both (a) horizontal navigation for long-duration balloon flights as well as (b) vertical scans over ranges of 10 to 20 kilometers below the float altitude of the long duration super pressure balloon platforms operating to altitudes up to 40 km.

\subsection{The StratoCruiser Observing System Concept.}

Long duration observing platforms operating in the stratosphere at altitudes between 20km and 40km provide critically needed scientific breakthroughs in both the Space Sciences and the Earth Sciences. The StratoCruiser Propulsion Module offers unprecedented mobility and measurement capability combining the persistence of balloon platforms for greatly extended observing times, station keeping over the central U.S. in July and August, and recovery of the experiment following the system deployment. The StratoCruiser long-duration observing system presented here engages the union of four separate advances in engineering, technology, and science: (1) the use of long-duration super-pressure balloon technology for flight durations of six weeks in the stratosphere at altitudes of 20 to 40 km, (2) a stratospheric solar-electric propulsion system for horizontal navigation and station keeping in the stratosphere that provides drive velocities up to 8 m/s, (3) a “reeldown” system providing in situ observations over an altitude range of 10 to 15km below the balloon float altitude, and finally (4) recognition and engagement of the unique anti-cyclonic flow in the lower stratosphere over the US in summer that provides to-this-point unrecognized opportunities for long duration flights of balloon platforms over the US.

In the course of presenting the dominant unanswered scientific questions addressing changes to the Earth’s climate, the StratoCruiser system provides, for the first time, observations with the following critical capabilities: 
    • the structure of the 3-D velocity fields within the global structure in the stratosphere,
    • the structure of the wave-breaking events associated with gravity waves, Coriolis control, stratosphere-troposphere exchange, as well as the impact of convective intrusion,
    • the concentration of species co-injected with water by convective events that are increasing in both intensity and frequency with the continued use of fossil fuels, 
    • both the vapor phase and condensed phase H2O and HDO isotopic concentrations as well as the full spectrum of atmospheric tracers convectively injected, 
    • the concentration of (a) the reactive chemical precursors that are normally removed by photolysis and oxidation in the troposphere, (b) chemical tracers injected by the convection, 
    • subsequent chemical kinetics of the injected chemical cocktail that tracks the time evolution of the source species, reactive intermediates, isotopes and catalytic free radicals that attack ozone, and 
    • direct detection of the structure and function of stratosphere-troposphere exchange that is a key diagnostic in tracing irreversible changes to the large-scale dynamical structure of the climate system in response to fossil fuel combustion products.
    
\subsection{Scientific Challenge: Changes to the Large-Scale Dynamical Structure of the Earth’s Climate System.}

The large-scale dynamical structure of the global atmosphere, displayed graphically in Figure 2, constitutes one of the most critical factors that determine the Earth’s response to increased forcing by fossil fuel extraction, distribution and combustion. The reason is that the large scale dynamical structure of the atmosphere determines: (1) the geographic position of deserts, of the tropics, and of the cryo-systems in the polar regions, (2) the geographic position and variance in the trajectory of the subtropical jet that determines storm intensity, weather pattern stability, rainfall and temperature extremes, as a function of season, (3) the trajectory of hurricanes, typhoons and large scale storm systems, and (4) the amount of water vapor entering and exiting the stratosphere that constitutes a critically important climate feedback as well as a key determinant that establishes the degree of global stratospheric ozone loss and thus of the amount of ultraviolet radiation reaching the Earth’s surface.

The new StratoCruiser observing system can systematically and comprehensively map the details of this dynamical structure globally employing an array of high spatial resolution in situ measurements of short, medium and long lived atmospheric tracers in combination with highly sensitive dynamical observations of three-dimensional velocity fields, wave-breaking structures, momentum transport and heat transport, as well as radiance divergence observations. These are the detailed, high spatial resolution observations that are critically needed to quantitatively establish the dynamical structure of the atmosphere required to develop tested and trusted forecast models of climate response to rapidly increased forcing by carbon dioxide and methane. Yet these observations have never been made because the critically important observing platform has not been available. Introduction of the StratoCruiser system will solve this problem.

As greenhouse gases increase in Earth’s atmosphere, the stratosphere is predicted to have two distinct responses. First, as the surface warms, the stratosphere cools, and both observations and models show that stratospheric cooling is a robust response to increasing radiative forcing by greenhouse gases. Second, chemistry-climate models universally predict that the Brewer-Dobson circulation (BDC) – the primary circulation pattern in the stratosphere – should be accelerating in response to greenhouse gas increases. The BDC is responsible for transporting trace gases, such as water vapor and ozone, that are critical for radiative forcing and impact surface weather and climate. Acceleration of the BDC predicted by models would be a positive feedback on the increased radiative forcing by greenhouse gases.

Quantifying how mean ages, residence times, and transport pathways vary with latitude and altitude is critical for understanding the Brewer-Dobson circulation and its role in controlling trace gas distributions. The StratoCruiser system will provide measurements of mean ages from CO2 and SF6, residence times from 14CO2, and age and pathway diagnostics from photolytic trace gas profiles of CFCs and other halocarbons,  including in the Southern Hemisphere. The StratoCruiser system will deliver transformative new observations and analyses quantifying trends in the BDC, ozone, and water vapor, and the degree to which we understand the mechanisms underlying these trends.  

\subsection{Scientific Challenge: Stratospheric ozone loss over the central United States in summer.}

    
    

==> Old_Files/Education_Outreach.tex <==


\chapter{Education \& Outreach}

In a December 2018 report by the Committee on STEM Education (COSTEM) of the National Science \& Technology Council, “Charting A Course for Success: America’s Strategy for STEM Education”, three major objectives were identified for NASA: 1) foster STEM ecosystems that unite communities, 2) increase work-based learning and training through educator-employer partnerships, and 3) encourage transdisciplinary learning. While ballooning contributes to all three objectives it is the last one where ballooning has the most impact on STEM education. In fact, the report highlighted a NASA balloon platform as an exemplary example of transdisciplinary learning (Figure~\ref{students}). Thus, in addition to supporting multiple significant scientific objectives, ballooning contributes to the aerospace workforce development pipeline, enhancing public awareness of NASA programs, and training the next generation of scientists and engineers.


\begin{figure*}[htb!]
\begin{center}
\centerline{\includegraphics[width=4.5in]{figures/studentBalloon.png}~~~~~\includegraphics[width=2in]{figures/moonShadow.png}}
\caption{\small \it Left: University students watching the launch of their experiments carried by a 
NASA balloon platform in September 2018. This program was highlighted in the recent COSTEM report as an exemplary example of transdisciplinary learning.
Right: Image of the moon’s shadow on the Earth during the solar eclipse of August 21, 2017 by the 
Montana State University student team balloon payload.
\label{students}}
\end{center}
\end{figure*}


\section{The Workforce Development Pipeline.}

Ballooning is a unique NASA capability that supports workforce development from K-12 through early career faculty and engineers. Scientific ballooning provides high quality, experiential projects for students from K-12 through graduate school that enables interdisciplinary STEM workforce training consistent with the COSTEM report objectives assigned to NASA. In addition, nation-wide programs making use of the established National Space Grant College and Fellowship network, provide special opportunities to not only support workforce development but to also convey the advantages of scientific ballooning to new and large audiences. 


\section{Enhance the Public Awareness of Ballooning.}

For the August 21, 2017 North America total solar eclipse 54 teams from 32 states involving over 900 students were positioned across the path of totality from Oregon to South Carolina and flew payloads to an altitude up to ~100,000 feet to downlink HD video of the moon’s shadow on Earth (see Figure 2) that was live streamed over the internet. This effort, organized by the Montana Space Grant Consortium was an amazing success and was featured as part of NASA’s eclipse coverage, which reached 600 million people. These kinds of projects engage the public, as well as students, exciting their imagination, and encouraging them to learn more about NASA ballooning. 


\section{Training Next Generation Scientists \& Engineers.}

Balloon platforms are a critical vehicle for supporting PI-class academic research due to the A) short time scale between conception and flight results, B) relatively low cost, and C) recoverability. This combination of characteristics enables universities to support research programs that develop near-space flight hardware while engaging future scientists and engineers. As most balloon experiments are recovered and reflown the acceptable risk on individual balloon payloads should be high relative to spacecraft. By accepting risk on balloon payloads, quality assurance requirements are reduced which, in turn, will decrease development time and overall cost.

\begin{figure}[htb!]
\begin{center}
\centerline{\includegraphics[width=5.in]{figures/moonShadow.png}}
\caption{\small \it Image of the moon’s shadow on the Earth during the solar eclipse of August 21, 2017 by the 
Montana State University student team balloon payload.
\label{moonshadow}}
\end{center}
\end{figure}

Recently, however, there is growing concern that safety and quality assurance requirements are increasing in the direction toward spacecraft mission requirements. If this trend is allowed to continue it is likely that the project time of development and cost will increase while access to the instrument by untrained students or early career faculty will decrease.  These trends would have an adverse impact on training the next generation of scientists and engineers. 



\section{Findings and recommendations for education and outreach.}

\begin{itemize}
\item
The PAG recommends that NASA should engage with the National Space Grant College and Fellowship program to continue and expand strong support for student training ballooning programs that support the workforce development pipeline at all levels including K-12, university students, and in-service teachers.

\item
Thus, the PAG recommends that NASA engage with stakeholders interested in the April 8, 2024 North American total solar eclipse as early as possible to assess scientific, workforce development, and public engagement projects, as well as payload weight classes including heavy payloads, and potential launch sites. 

\item
The PAG recommends that balloon project safety and performance standards be reviewed at a level significantly below spacecraft standards, be relevant to the project, avoid duplication of effort, be consistent with the need to provide novice personnel the flexibility to have direct involvement in the payload success, and be associated with relevant, simple, concise, and straight forward best practices and safety training materials.
\end{itemize}


